Time Calibration of the Baikal-GVD Neutrino Telescope with Atmospheric Muons

We present a new procedure for time calibration of the Baikal-GVD neutrino telescope. The track reconstruction quality depends on accurate measurements of arrival times of Cherenkov photons. Therefore, it is crucial to achieve a high precision in time calibration. For that purpose, in addition to other calibration methods, we employ a new procedure using atmospheric muons reconstructed in a single-cluster mode. The method is based on iterative determination of effective time offsets for each optical module. This paper focuses on the results of the iterative reconstruction procedure with time offsets from the previous iteration and the verification of the method developed. The theoretical muon calibration precision is estimated to be around 1.5-1.6ns.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

